GlossyGS: Inverse Rendering of Glossy Objects with 3D Gaussian Splatting

Reconstructing objects from posed images is a crucial and complex task in computer graphics and computer vision. While NeRF-based neural reconstruction methods have exhibited impressive reconstruction ability, they tend to be time-comsuming. Recent strategies have adopted 3D Gaussian Splatting (3D-GS) for inverse rendering, which have led to quick and effective outcomes. However, these techniques generally have difficulty in producing believable geometries and materials for glossy objects, a challenge that stems from the inherent ambiguities of inverse rendering. To address this, we introduce GlossyGS, an innovative 3D-GS-based inverse rendering framework that aims to precisely reconstruct the geometry and materials of glossy objects by integrating material priors. The key idea is the use of micro-facet geometry segmentation prior, which helps to reduce the intrinsic ambiguities and improve the decomposition of geometries and materials. Additionally, we introduce a normal map prefiltering strategy to more accurately simulate the normal distribution of reflective surfaces. These strategies are integrated into a hybrid geometry and material representation that employs both explicit and implicit methods to depict glossy objects. We demonstrate through quantitative analysis and qualitative visualization that the proposed method is effective to reconstruct high-fidelity geometries and materials of glossy objects, and performs favorably against state-of-the-arts.

==> figonly1.tex <==
\clearpage

\begin{figure*}[p]
\begin{center}
    \addtolength{\tabcolsep}{-4pt}
    \begin{tabular}{m{2.5cm}<{\centering} m{2.5cm}<{\centering} m{2.5cm}<{\centering} m{2.5cm}<{\centering} m{2.5cm}<{\centering} m{2.5cm}<{\centering}m{2.5cm}<{\centering}}
    
    Scene & NeRO & NMF & Gshader & GSIR &Ours & GT \\
    \includegraphics[width=0.9in]{figures/experiment/normalcompare/car2/gt_00120.png} &
    \includegraphics[width=0.9in]{figures/experiment/normalcompare/car2/nero_normal_00120.png} &
    \includegraphics[width=0.9in]{figures/experiment/normalcompare/car2/nmf_normal_00120.png} &
    \includegraphics[width=0.9in]{figures/experiment/normalcompare/car2/gshader_normal_00120.png} &
    \includegraphics[width=0.9in]{figures/experiment/normalcompare/car2/gsir_normal_00120.png} &
    \includegraphics[width=0.9in]{figures/experiment/normalcompare/car2/ours_normal_00120.png} &
    \includegraphics[width=0.9in]{figures/experiment/normalcompare/car2/gt_normal_00120.png} \\
    Car & & & & & & \\
    % \includegraphics[height=1in]{figures/experiment/normalcompare/toaster/00181.png} &
    % \includegraphics[height=1in]{figures/experiment/normalcompare/toaster/nero_normal_00181.png} &
    % \includegraphics[height=1in]{figures/experiment/normalcompare/toaster/nmf_normal_00181.png} &
    % \includegraphics[height=1in]{figures/experiment/normalcompare/toaster/gshader_00181.png} &
    % \includegraphics[height=1in]{figures/experiment/normalcompare/toaster/gsir_normal_00181.png} &
    % \includegraphics[height=1in]{figures/experiment/normalcompare/toaster/ours_normal_00181.png} &
    % \includegraphics[height=1in]{figures/experiment/normalcompare/toaster/gt_normal_00181.png} \\
    % % Toaster & & & & & & \\
    \includegraphics[height=1in]{figures/experiment/normalcompare/luyu/00005.png} &
    \includegraphics[height=1in]{figures/experiment/normalcompare/luyu/nero_normal_00005.png} &
    \includegraphics[height=1in]{figures/experiment/normalcompare/luyu/nmf_00005.png} &
    \includegraphics[height=1in]{figures/experiment/normalcompare/luyu/gshader_00005.png} &
    \includegraphics[height=1in]{figures/experiment/normalcompare/luyu/gsir_normal_00005.png} &
    \includegraphics[height=1in]{figures/experiment/normalcompare/luyu/ours_normal_00005.png} &
    \resizebox{0.2\columnwidth}{!}{N/A} \\
    Luyu & & & & & & \\
    
    \includegraphics[height=1in]{figures/experiment/normalcompare/angel/gt_00000.png} &
    \includegraphics[height=1in]{figures/experiment/normalcompare/angel/nero_normal_00000.png} &
    \includegraphics[height=1in]{figures/experiment/normalcompare/angel/nmf_00000.png} &
    \includegraphics[height=1in]{figures/experiment/normalcompare/angel/gshader_00000.png} &
    \includegraphics[height=1in]{figures/experiment/normalcompare/angel/gsir_normal_00000.png} &
    \includegraphics[height=1in]{figures/experiment/normalcompare/angel/ours_normal_00000.png} &
    \resizebox{0.2\columnwidth}{!}{N/A} \\
    Angel & & & & & & \\
    \end{tabular}
\end{center}
\caption{Comparison of normal reconstruction among our method, NMF~\cite{mai2023neural}, NeRO \cite{liu2023nero}, Gshader \cite{jiang2023gaussianshader} and GSIR \cite{liang2023gs} on the Shiny Blender \cite{verbin2022ref} (the first rows), Glossy Synthetic  datasets \cite{liu2023nero}(the second and third rows). Note that there is no available ground-truth normal in the Glossy Synthetic dataset.}
\label{fig:normal_syn}
\end{figure*}

\begin{figure*}[p]
\begin{center}
    % \addtolength{\tabcolsep}{-4pt}
    % \begin{tabular}{cccccccc}
        \addtolength{\tabcolsep}{-4pt}
    \begin{tabular}{m{2.5cm}<{\centering} m{2.5cm}<{\centering} m{2.5cm}<{\centering} m{2.5cm}<{\centering} m{2.5cm}<{\centering} m{2.5cm}<{\centering}m{2.5cm}<{\centering}}
    
    Scene & NeRO albedo & GSIR albedo & Our albedo &  Our metallic & Our roughness & Our relighting\\
    \includegraphics[width=1in]{figures/experiment/decompo/ball/gt_00039.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/ball/nero_diffuse_00039.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/ball/gsir_diffuse_00039.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/ball/ours_diffuse2_00039.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/ball/ours_metallic_00039.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/ball/ours_roughness_00039.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/00039_city.png}
    % \includegraphics[width=1in]{figures/experiment/decompo/seg/r_43.jpg_sam_bgwhite.jpg}
    % \includegraphics[width=1in]{figures/experiment/decompo/relight/00039_sunset (1).png}
    \\
    % Ball  & & & & & & \\
    
    \includegraphics[width=1in]{figures/experiment/decompo/toaster/gt_00030.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/toaster/nero_diffuse_00030.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/toaster/gsir_diffuse_00030.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/toaster/ours_diffuse2_00030.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/toaster/ours_metallic_00030.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/toaster/ours_roughness_00030.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/00030_provence_studio_1k (1).png}\\
    % \includegraphics[width=1in]{figures/experiment/decompo/seg/r_30.jpg_sam_bgwhite.jpg}\\
    
    % Toaster  & & & & & & \\
    
    \includegraphics[width=1in]{figures/experiment/decompo/car/gt_00028.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/car/nero_diffuse_00028.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/car/gsir_diffuse_00028.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/car/ours_diffuse2_00028.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/car/ours_metallic_00028.png} &
    \includegraphics[width=1in]{figures/experiment/decompo/car/ours_roughness_00028.png}  &
    \includegraphics[width=1in]{figures/experiment/decompo/00028_hall (1).png} \\
    % \includegraphics[height=0.5in]{figures/experiment/decompo/seg/r_51.jpg_sam_bgwhite (1).jpg}\\

    % Car  & & & & & & \\
    \end{tabular}
\end{center}
\caption{Comparison of the estimated BRDFs among our method, NeRO \cite{liu2023nero} and GSIR \cite{liang2023gs}.}
\label{fig:material}
\end{figure*}


\begin{figure*}[p]
\begin{center}
    \addtolength{\tabcolsep}{-4pt}
    \begin{tabular}{ccccc}
    
    Scene & Gshader & GSIR &Ours & Reference \\
    \includegraphics[height=0.7in]{figures/experiment/envmap/gt_teapot.png} &
    \includegraphics[height=0.7in]{figures/experiment/envmap/gshader_teapot.jpg} &
    \includegraphics[height=0.7in]{figures/experiment/envmap/teapot_gsirenvmap.png} &
    \includegraphics[height=0.7in]{figures/experiment/envmap/teapot_light.jpeg}&
    \includegraphics[height=0.7in]{figures/experiment/envmap/teapot_gt.jpeg}\\
    
    \includegraphics[height=0.7in]{figures/experiment/envmap/gt_angel.png}  &
    \includegraphics[height=0.7in]{figures/experiment/envmap/gshader_angel.png} &
    \includegraphics[height=0.7in]{figures/experiment/envmap/angel_gsir.png} &
    \includegraphics[height=0.7in]{figures/experiment/envmap/angel_light.jpeg}&
    \includegraphics[height=0.7in]{figures/experiment/envmap/angel_gt.jpeg}\\
    
    
    
    \end{tabular}
\end{center}
\caption{Comparison of environment maps among our method, Gshader \cite{jiang2023gaussianshader} and GSIR \cite{liang2023gs}.}
\label{fig:envmap}
\end{figure*}


==> figonly_old.tex <==
\clearpage



\begin{figure*}[p]
\begin{center}
    \addtolength{\tabcolsep}{-4pt}
    \begin{tabular}{m{2.5cm}<{\centering} m{2.5cm}<{\centering} m{2.5cm}<{\centering} m{2.5cm}<{\centering} m{2.5cm}<{\centering} m{2.5cm}<{\centering}m{2.5cm}<{\centering}}
    
    Scene & TensoIR & NeRO & Gshader & GSIR &Ours & GT \\
    \includegraphics[height=0.6in]{figures/experiment/normalcompare/car/00146.png} &
    \includegraphics[height=0.6in]{figures/experiment/normalcompare/car/tensoir_normal_00146.png} &
    \includegraphics[height=0.6in]{figures/experiment/normalcompare/car/nero_normal_00146.png} &
    \includegraphics[height=0.6in]{figures/experiment/normalcompare/car/gshader_00146.png} &
    \includegraphics[height=0.6in]{figures/experiment/normalcompare/car/gsir_normal_00146.png} &
    \includegraphics[height=0.6in]{figures/experiment/normalcompare/car/ours_normal_00146.png} &
    \includegraphics[height=0.6in]{figures/experiment/normalcompare/car/gt_normal_00146.png} \\
    
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/toaster/00181.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/toaster/tensoir_normal_00181.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/toaster/nero_normal_00181.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/toaster/gshader_00181.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/toaster/gsir_normal_00181.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/toaster/ours_normal_00181.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/toaster/gt_normal_00181.png} \\
    % Toaster & & & & & & \\
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/luyu/00005.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/luyu/tensoir_normal_00005.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/luyu/nero_normal_00005.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/luyu/gshader_00005.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/luyu/gsir_normal_00005.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/luyu/ours_normal_00005.png} &
    \resizebox{0.2\columnwidth}{!}{N/A} \\
    % Luyu & & & &  \\
    
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/angel/gt_00000.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/angel/tensoir_normal_00000.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/angel/nero_normal_00000.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/angel/gshader_00000.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/angel/gsir_normal_00000.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/angel/ours_normal_00000.png} &
    \resizebox{0.2\columnwidth}{!}{N/A} \\
    % Angel & & & &  \\
    
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/cactus/crop3/0062.png}  &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/cactus/crop3/tensoir_normal_00002.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/cactus/crop3/nero_normal_00002.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/cactus/crop3/shader00002.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/cactus/crop3/gsir_normal_00002.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/cactus/crop3/ours_normal00002.png}&
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/cactus/crop3/gt_normal_00002.png}\\
    
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/teapot2/crop2/0067.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/teapot2/crop2/tensoir_normal_00006.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/teapot2/crop2/nero_normal_00006.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/teapot2/crop2/gshader_00006.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/teapot2/crop2/gsir_normal_00006.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/teapot2/crop2/ours_normal00006.png} &
    \includegraphics[height=0.8in]{figures/experiment/normalcompare/teapot2/crop2/gt_normal_00006.png}\\
    \end{tabular}
\end{center}
\vspace{-0.15cm}
\caption{Comparison of normal reconstruction among our method, TensoIR \cite{jin2023tensoir}, NeRO \cite{liu2023nero}, Gshader \cite{jiang2023gaussianshader} and GSIR \cite{liang2023gs} on the Shiny Blender \cite{verbin2022ref} (the first and second rows), Glossy Synthetic \cite{liu2023nero} (the third and fourth rows) and Stanford-ORB datasets \cite{kuang2024stanford} (the fifth and sixth rows). Note that there is no available ground-truth normal in the Glossy Synthetic dataset.}
\label{fig:normal}
\end{figure*}



\begin{figure*}[p]
\begin{center}
    \addtolength{\tabcolsep}{-4pt}
    \begin{tabular}{m{2.916cm}<{\centering} m{2.916cm}<{\centering} m{2.916cm}<{\centering} m{2.916cm}<{\centering} m{2.916cm}<{\centering} m{2.916cm}<{\centering}}
    
    TensoIR & NeRO & Gshader & GSIR & Ours &GT \\
    \includegraphics[height=0.6in]{figures/experiment/nvs/tbell/tensoir_00003.png} &
    \includegraphics[height=0.6in]{figures/experiment/nvs/tbell/nero_pred_00003.png} &
    \includegraphics[height=0.6in]{figures/experiment/nvs/tbell/gshader_00003.png} &
    \includegraphics[height=0.6in]{figures/experiment/nvs/tbell/gsir_00003.png} &
    \includegraphics[height=0.6in]{figures/experiment/nvs/tbell/ours_pred_00003.png}&
    \includegraphics[height=0.6in]{figures/experiment/nvs/tbell/gt_00003.png} \\
     % &28.93& & 22.21 &30.48& Tbell
    
    % \includegraphics[height=1.1in]{figures/experiment/nvs/car/tensoir_00009.png} &
    % \includegraphics[height=1.1in]{figures/experiment/nvs/car/nero_pred_00009.png} &
    % \includegraphics[height=1.1in]{figures/experiment/nvs/car/gshader_00009.png} &
    % \includegraphics[height=1.1in]{figures/experiment/nvs/car/gsir_00009.png} &
    % \includegraphics[height=1.1in]{figures/experiment/nvs/car/00009.png} &
    % \includegraphics[height=1.1in]{figures/experiment/nvs/car/gt_00009.png}\\

    \includegraphics[height=0.55in]{figures/experiment/nvs/grogu/tensoir_pred_00000.png} &
    \includegraphics[height=0.55in]{figures/experiment/nvs/grogu/nero_pred_00000.png} &
    \includegraphics[height=0.55in]{figures/experiment/nvs/grogu/gshader_00000.png} &
    \includegraphics[height=0.55in]{figures/experiment/nvs/grogu/gsir_pred_00000.png} &
    \includegraphics[height=0.55in]{figures/experiment/nvs/grogu/ours_pred_00000.png} &
    \includegraphics[height=0.55in]{figures/experiment/nvs/grogu/gt_00000.png}\\
    % &27.08 & & 37.77 &36.05 & Grogu \\
    
    % \includegraphics[height=0.8in]{figures/experiment/nvs/teapot/tensoir_pred_00004.png} &
    % \includegraphics[height=0.8in]{figures/experiment/nvs/teapot/nero_pred_00004.png} &
    % \includegraphics[height=0.8in]{figures/experiment/nvs/teapot/gshader_00004.png} &
    % \includegraphics[height=0.8in]{figures/experiment/nvs/teapot/gsir_pred_00004.png} &
    % \includegraphics[height=0.8in]{figures/experiment/nvs/teapot/ours.png} &
    % \includegraphics[height=0.8in]{figures/experiment/nvs/teapot/gt_00004.png}\\
    
    
    \end{tabular}
\end{center}
\vspace{-0.5cm}
\caption{Comparison of novel view synthesis among our method, TensoIR \cite{jin2023tensoir}, NeRO \cite{liu2023nero}, Gshader \cite{jiang2023gaussianshader} and GSIR \cite{liang2023gs}.}
\vspace{-0.3cm}
\label{fig:nvs}
\end{figure*}

% \begin{figure*}[p]
% \begin{center}
%     \addtolength{\tabcolsep}{-4pt}
%     \begin{tabular}{ccccccc}
    
%     Scene & TensoIR & NeRO & Gshader & GSIR &Ours & GT \\
%     \includegraphics[height=0.8in]{figures/experiment/normalcompare/cactus/crop3/0062.png}  &
%     \includegraphics[height=0.8in]{figures/experiment/normalcompare/cactus/crop3/tensoir_normal_00002.png} &
%     \includegraphics[height=0.8in]{figures/experiment/normalcompare/cactus/crop3/nero_normal_00002.png} &
%     \includegraphics[height=0.8in]{figures/experiment/normalcompare/cactus/crop3/shader00002.png} &
%     \includegraphics[height=0.8in]{figures/experiment/normalcompare/cactus/crop3/gsir_normal_00002.png} &
%     \includegraphics[height=0.8in]{figures/experiment/normalcompare/cactus/crop3/ours_normal00002.png}&
%     \includegraphics[height=0.8in]{figures/experiment/normalcompare/cactus/crop3/gt_normal_00002.png}\\
    
%     \includegraphics[height=0.8in]{figures/experiment/normalcompare/teapot2/crop2/0067.png} &
%     \includegraphics[height=0.8in]{figures/experiment/normalcompare/teapot2/crop2/nero_normal_00006.png} &
%     \includegraphics[height=0.8in]{figures/experiment/normalcompare/teapot2/crop2/nero_normal_00006.png} &
%     \includegraphics[height=0.8in]{figures/experiment/normalcompare/teapot2/crop2/gshader_00006.png} &
%     \includegraphics[height=0.8in]{figures/experiment/normalcompare/teapot2/crop2/gsir_normal_00006.png} &
%     \includegraphics[height=0.8in]{figures/experiment/normalcompare/teapot2/crop2/ours_normal00006.png} &
%     \includegraphics[height=0.8in]{figures/experiment/normalcompare/teapot2/crop2/gt_normal_00006.png}\\
    
    
%     \end{tabular}
% \end{center}
% \caption{Comparison of the geometry reconstruction between our method and NeRO \cite{liu2023nero} on Stanford-ORB dataset \cite{kuang2024stanford}.}
% \label{fig:normal_stanfordorb}
% \end{figure*}





% \begin{figure*}[p]
% \begin{center}
%     \addtolength{\tabcolsep}{-4pt}
%     \begin{tabular}{cccccc}
    
%     Scene & TensoIR & NeRO & Gshader & GSIR &Ours \\
%     % \includegraphics[height=1.1in]{figures/experiment/normalcompare/luyu/00003.png} &
%     % \includegraphics[height=1.1in]{figures/experiment/normalcompare/luyu/tensoir_normal_00003.png} &
%     % \includegraphics[height=1.1in]{figures/experiment/normalcompare/luyu/nero_normal_00003.png} &
%     % \includegraphics[height=1.1in]{figures/experiment/normalcompare/luyu/gshader_00003.png} &
%     % \includegraphics[height=1.1in]{figures/experiment/normalcompare/luyu/gsir_normal_00003.png} &
%     % \includegraphics[height=1.1in]{figures/experiment/normalcompare/luyu/ours_normal_00003.png}\\
%     % % 
    
    
%     % \includegraphics[height=1.3in]{figures/experiment/normalcompare/teapot/gt_00004.png} &
%     % \includegraphics[height=1.3in]{figures/experiment/normalcompare/teapot/nero_normal_00004.png} &
%     % \includegraphics[height=1.3in]{figures/experiment/normalcompare/teapot/gsahder_normal00004.png} &
%     % \includegraphics[height=1.3in]{figures/experiment/normalcompare/teapot/gsir_normal_00004.png} &
%     % \includegraphics[height=1.3in]{figures/experiment/normalcompare/teapot/ours_normal00004.png}\\
    
    
%     \end{tabular}
% \end{center}
% \caption{Comparison of geometry reconstruction among our method, TensoIR \cite{jin2023tensoir}, NeRO \cite{liu2023nero}, Gshader \cite{jiang2023gaussianshader} and GSIR \cite{liang2023gs} on Glossy Synthetic dataset \cite{liu2023nero}. There is no available ground-truth normal in the dataset.}
% \label{fig:normal_nero}
% \end{figure*}


\begin{figure*}[p]
\begin{center}
        \addtolength{\tabcolsep}{-4pt}
    \begin{tabular}{m{2.1875cm}<{\centering} m{2.1875cm}<{\centering} m{2.1875cm}<{\centering} m{2.1875cm}<{\centering} | m{2.1875cm}<{\centering} m{2.1875cm}<{\centering}m{2.1875cm}<{\centering} m{2.1875cm}<{\centering}}
    
    NeRO  & GSIR &Ours & GT & NeRO  & GSIR &Ours & GT \\
    % \includegraphics[height=1.1in]{figures/experiment/relight/cactus2/nero_pred_00002.png} &
    % \includegraphics[height=1.1in]{figures/experiment/relight/cactus2/gshader_pred_00002.png} &
    % \includegraphics[height=1.1in]{figures/experiment/relight/cactus2/gsir_pred_00002.png} &
    % \includegraphics[height=1.1in]{figures/experiment/relight/cactus2/ours_pred_00002.png}&
    % \includegraphics[height=1.1in]{figures/experiment/relight/cactus2/gt_00002.png} \\
    
    \includegraphics[height=0.5in]{figures/experiment/relight/teapot/crop/nero_pred_00003.png} &
    % \includegraphics[height=0.7in]{figures/experiment/relight/teapot/crop/gshader00003.png} &
    \includegraphics[height=0.5in]{figures/experiment/relight/teapot/crop/gsir_pred_00003.png} &
    \includegraphics[height=0.5in]{figures/experiment/relight/teapot/crop/ours_pred_00003.png} &
    \includegraphics[height=0.5in]{figures/experiment/relight/teapot/crop/gt_00003.png} &  
    
    \includegraphics[height=0.44in]{figures/experiment/relight/grogu/nero_pred_00015.png} &
    % \includegraphics[height=0.6in]{figures/experiment/relight/grogu/gshader_pred_00015.png} &
    \includegraphics[height=0.44in]{figures/experiment/relight/grogu/gsir_pred_00015.png} &
    \includegraphics[height=0.44in]{figures/experiment/relight/grogu/ours_pred_00015.png} &
    \includegraphics[height=0.44in]{figures/experiment/relight/grogu/gt_00015.png}\\


    % \includegraphics[height=0.6in]{figures/experiment/relight/grogu2/nero_pred_00000.png} &
    % \includegraphics[height=0.6in]{figures/experiment/relight/grogu2/gshader_pred_00000.png} &
    % \includegraphics[height=0.6in]{figures/experiment/relight/grogu2/gsir_pred_00000.png} &
    % \includegraphics[height=0.6in]{figures/experiment/relight/grogu2/ours_pred_00000.png} &
    % \includegraphics[height=0.6in]{figures/experiment/relight/grogu2/gt_00000.png}\\\\
    
    
    \end{tabular}
\end{center}
\vspace{-0.4cm}
\caption{Comparison of relighting among our method, NeRO \cite{liu2023nero} and GSIR \cite{liang2023gs} on the Stanford-ORB \cite{kuang2024stanford} dataset.}
\label{fig:relight_stanfordorb}
\vspace{-0.3cm}
\end{figure*}


\begin{figure*}[p]
\begin{center}
    \addtolength{\tabcolsep}{-4pt}
    \begin{tabular}{m{2.916cm}<{\centering} m{2.916cm}<{\centering} m{2.916cm}<{\centering} m{2.916cm}<{\centering} m{2.916cm}<{\centering} m{2.916cm}<{\centering}}
    
    New lights & NeRO & Gshader& GSIR &Ours  & GT\\
    \centering
    \includegraphics[height=0.5in]{figures/experiment/relight/golf.jpg} &
    \includegraphics[height=0.8in]{figures/experiment/relight/angel/nero_pred_00017.png} &
    \includegraphics[height=0.8in]{figures/experiment/relight/angel/gshader_pred_00017.png} &
    \includegraphics[height=0.8in]{figures/experiment/relight/angel/gsir_pred_00017.png} &
    \includegraphics[height=0.8in]{figures/experiment/relight/angel/ours_pred_00017.png} &
    \includegraphics[height=0.8in]{figures/experiment/relight/angel/gt_00017.png}\\
    
    % \includegraphics[height=0.4in]{figures/experiment/relight/neon.jpg} &
    % \includegraphics[height=1.3in]{figures/experiment/relight/horse/nero_pred_00035.png} &
    % \includegraphics[height=1.3in]{figures/experiment/relight/horse/gshader_pred_00035.png} &
    % \includegraphics[height=1.3in]{figures/experiment/relight/horse/gsir_pred_00035.png} &
    % \includegraphics[height=1.3in]{figures/experiment/relight/horse/ours_pred_00035.png} &
    % \includegraphics[height=1.3in]{figures/experiment/relight/horse/gt_00035.png} \\

    \includegraphics[height=0.5in]{figures/experiment/relight/corridor.jpg} &
    \includegraphics[height=1in]{figures/experiment/relight/horse2/nero_pred_00000.png} &
    \includegraphics[height=1in]{figures/experiment/relight/horse2/gshader_pred_00000.png} &
    \includegraphics[height=1in]{figures/experiment/relight/horse2/gsir_pred_00000.png} &
    \includegraphics[height=1in]{figures/experiment/relight/horse2/ours_pred_00000.png} &
    \includegraphics[height=1in]{figures/experiment/relight/horse2/gt_00000.png} \\

    
    \includegraphics[height=0.5in]{figures/experiment/relight/golf.jpg} &
    \includegraphics[height=0.8in]{figures/experiment/relight/luyu/nero_pred_00021.png} &
    \includegraphics[height=0.8in]{figures/experiment/relight/luyu/gshader_pred_00021.png} &
    \includegraphics[height=0.8in]{figures/experiment/relight/luyu/gsir_pred_00021.png} &
    \includegraphics[height=0.8in]{figures/experiment/relight/luyu/ours_pred_00021.png} &
    \includegraphics[height=0.8in]{figures/experiment/relight/luyu/gt_00021.png} \\
    
    
    \end{tabular}
\end{center}
\vspace{-0.5cm}
\caption{Comparison of relighting results among our method, NeRO \cite{liu2023nero}, Gshader \cite{jiang2023gaussianshader} and GSIR \cite{liang2023gs} on the Glossy Synthetic dataset \cite{liu2023nero}.}
\label{fig:relight_nero}
\vspace{-0.4cm}
\end{figure*}







\begin{figure*}[p]
\begin{center}
    \addtolength{\tabcolsep}{-4pt}
    \begin{tabular}{m{2.916cm}<{\centering} m{2.916cm}<{\centering} m{2.916cm}<{\centering} m{2.916cm}<{\centering} | m{2.916cm}<{\centering} m{2.916cm}<{\centering}}
    
    Scene & Gshader & GSIR &Ours & Our relighting & Segment prior \\
    % \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/gt_womask_00042.png} &
    % \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/00042gshader.png} &
    % \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/00042gsir.png} &
    % \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/oursnormal.png}&
    % \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/00071.png} &
    % \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/042_sam.jpeg} \\

    
    % % \includegraphics[height=1.1in]{figures/experiment/dtu/qilin/gt_womask_00012.png} &
    % % \includegraphics[height=1.1in]{figures/experiment/dtu/qilin/gshader_00012.png} &
    % % \includegraphics[height=1.1in]{figures/experiment/dtu/qilin/gsir-00012.png} &
    % % \includegraphics[height=1.1in]{figures/experiment/dtu/qilin/00010.png}&
    % % \includegraphics[height=1.1in]{figures/experiment/dtu/qilin/00010_hotel_room_1k.png} &
    % % \includegraphics[height=1.1in]{figures/experiment/dtu/qilin/00010_interior.png} \\
    
    % \includegraphics[height=1.1in]{figures/experiment/dtu/53brass/gt_womask_00053.png} &
    % \includegraphics[height=1.1in]{figures/experiment/dtu/53brass/gshader_00053.png} &
    % \includegraphics[height=1.1in]{figures/experiment/dtu/53brass/gsir00053.png} &
    % \includegraphics[height=1.1in]{figures/experiment/dtu/53brass/ours-00053.png}&
    % \includegraphics[height=1.1in]{figures/experiment/dtu/brass0519/00048.png} &
    % \includegraphics[height=1.1in]{figures/experiment/dtu/53brass/053_sam_bgwhite (1).jpg} \\


            
        \includegraphics[height=1.1in]{figures/experiment/dtu/53brass/gt_womask_00053.png} &
    \includegraphics[height=1.1in]{figures/experiment/dtu/53brass/gshader_00053.png} &
    \includegraphics[height=1.1in]{figures/experiment/dtu/53brass/gsir00053.png} &
    \includegraphics[height=1.1in]{figures/experiment/dtu/53brass/ours-00053.png}&
    \includegraphics[height=1.1in]{figures/experiment/dtu/brass0519/00048.png} &
    \includegraphics[height=1.1in]{figures/experiment/dtu/53brass/053_sam_bgwhite (1).jpg} \\

    \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/gt_womask_00042.png} &
    \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/00042gshader.png} &
    \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/00042gsir.png} &
    \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/oursnormal.png}&
    \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/00071.png} &
    % \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/00039.png} &
            \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/042_sam_new.jpeg}\\
    
    % \includegraphics[height=1.1in]{figures/experiment/dtu/89brass/gt_womask_00089.png} &
    % \includegraphics[height=1.1in]{figures/experiment/dtu/89brass/gshader00089.png} &
    % \includegraphics[height=1.1in]{figures/experiment/dtu/89brass/gsir00089.png} &
    % \includegraphics[height=1.1in]{figures/experiment/dtu/89brass/ours00089.png}&
    % \includegraphics[height=1.1in]{figures/experiment/dtu/89brass/00089_hotel_room_1k.png} &
    % \includegraphics[height=1.1in]{figures/experiment/dtu/89brass/00089_factory.png} \\
    
    
    \end{tabular}
\end{center}
\vspace{-0.5cm}
\caption{Comparison of normal reconstruction and relighting results among our method, Gshader \cite{jiang2023gaussianshader} and GSIR \cite{liang2023gs} on the NEILF-HDR \cite{zhang2023neilf++} dataset.}
\label{fig:neilf}
\end{figure*}




% \begin{figure*}[p]
% \begin{center}
%     \addtolength{\tabcolsep}{-4pt}
%     \begin{tabular}{m{2.5cm}<{\centering} m{2.5cm}<{\centering} m{2.5cm}<{\centering} m{2.5cm}<{\centering} m{2.5cm}<{\centering} m{2.5cm}<{\centering}m{2.5cm}<{\centering}}
    
%     Scene & Gshader & GSIR &Ours & Our relighting 1 & Our relighting 2 & Segment prior \\
%     % \includegraphics[height=1.1in]{figures/experiment/dtu/cat/005.png} &
%     % \includegraphics[height=1.1in]{figures/experiment/dtu/cat/00005gshader.png} &
%     % \includegraphics[height=1.1in]{figures/experiment/dtu/cat/00005gsir.png} &
%     % \includegraphics[height=1.1in]{figures/experiment/dtu/cat/00044-oursnormal.png}&
%     % \includegraphics[height=1.1in]{figures/experiment/dtu/cat/00036.png} &
%     % \includegraphics[height=1.1in]{figures/experiment/dtu/cat/00044.png} &
%     % \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/042_sam.jpeg}
%     % \\
%     % \includegraphics[height=1.1in]{figures/experiment/dtu/cat46/gt_womask_00046.png} &
%     % \includegraphics[height=1.1in]{figures/experiment/dtu/cat46/00046gshader.png} &
%     % \includegraphics[height=1.1in]{figures/experiment/dtu/cat46/00046gsir.png} &
%     % \includegraphics[height=1.1in]{figures/experiment/dtu/cat46/oursnormal.png}&
%     % \includegraphics[height=1.1in]{figures/experiment/dtu/cat46/00069.png} &
%     % \includegraphics[height=1.1in]{figures/experiment/dtu/cat46/00043-46.png} &
%     %     \includegraphics[height=1.1in]{figures/experiment/dtu/cat46/046_sam.jpeg}\\

    
%     \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/gt_womask_00042.png} &
%     \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/00042gshader.png} &
%     \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/00042gsir.png} &
%     \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/oursnormal.png}&
%     \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/00055.png} &
%     % \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/00039.png} &
%             \includegraphics[height=1.1in]{figures/experiment/dtu/cat42/042_sam_new.jpeg}\\
            
%         \includegraphics[height=1.1in]{figures/experiment/dtu/53brass/gt_womask_00053.png} &
%     \includegraphics[height=1.1in]{figures/experiment/dtu/53brass/gshader_00053.png} &
%     \includegraphics[height=1.1in]{figures/experiment/dtu/53brass/gsir00053.png} &
%     \includegraphics[height=1.1in]{figures/experiment/dtu/53brass/ours-00053.png}&
%     \includegraphics[height=1.1in]{figures/experiment/dtu/brass0519/00048.png} &
%         \includegraphics[height=1.1in]{figures/experiment/dtu/brass0519/00034.png} &
%     \includegraphics[height=1.1in]{figures/experiment/dtu/53brass/053_sam_bgwhite (1).jpg} \\
    
    
%     \end{tabular}
% \end{center}
% \vspace{-0.5cm}
% \caption{Comparison of normal reconstruction and relighting results among our method, Gshader \cite{jiang2023gaussianshader} and GSIR \cite{liang2023gs} on the NEILF-HDR \cite{zhang2023neilf++} dataset.}
% \label{fig:neilf}
% \end{figure*}
